MaxRay: A Raytracing-based Integrated Sensing and Communication Framework

Integrated Sensing And Communication (ISAC)forms a symbiosis between the human need for communication and the need for increasing productivity, by extracting environmental information leveraging the communication network. As multiple sensory already create a perception of the environment, an investigation into the advantages of ISAC compare to such modalities is required. Therefore, we introduce MaxRay, an ISAC framework allowing to simulate communication, sensing, and additional sensory jointly. Emphasizing the challenges for creating such sensing networks, we introduce the required propagation properties for sensing and how they are leveraged. To compare the performance of the different sensing techniques, we analyze four commonly used metrics used in different fields and evaluate their advantages and disadvantages for sensing. We depict that a metric based on prominence is suitable to cover most algorithms. Further we highlight the requirement of clutter removal algorithms, using two standard clutter removal techniques to detect a target in a typical industrial scenario. In general a versatile framework, allowing to create automatically labeled datasets to investigate a large variety of tasks is demonstrated.

==> pdfs/foo.tex <==
asd

==> tex_content/notations.tex <==
\chapter*{Notations \label{chap:Notations}}

\addcontentsline{toc}{chapter}{Notations}
\markboth{Notations}{Notations}
\setlength\extrarowheight{1em}
\begin{flushleft}
	\begin{longtable}{>{\raggedright}p{0.3\textwidth} >{\raggedright}p{0.69\textwidth}}
	$x$ & scalar variables, especially in time domain: italic lower case letters
	\tabularnewline
	$\mathbf{X}$ & matrix variables: boldface upright upper case letters
	\tabularnewline	
	$x\left(t\right)$ & functions of continuous variables: argument is placed in round parentheses
	\tabularnewline
	$x_{k}$ & scalar elements of a vector or element of a sequence: element index is a subscript
	\tabularnewline
	$X_{ij}$ & scalar elements of a matrix: row and column indices are subscripts
	\tabularnewline
	$\oplus$  & exclusive disjunction (xor)
	\tabularnewline
	$x \ast h $        & convolution of $x$ and $h$
	\tabularnewline
	$P[x<X]$         & probability of $x$ being smaller than $X$
	\tabularnewline
	$\mathbb{E}[X]$         & expected value of $X$
	\tabularnewline
	$\bf{H} \odot \bf{I}$      & Hadamard product of matrix $\bf{H}$ and $\bf{I}$ 
	\tabularnewline
	$j$       & imaginary unit
	\tabularnewline
	$<.>$     & Iverson brackets, turning the statement into Boolean
	\tabularnewline
	$\bf{H}^{\dagger}$ & pseudo inverse of $\bf{H}$
	\end{longtable}
	\par
\end{flushleft}
\setlength\extrarowheight{0em}


==> tex_content/plotcyclelists.tex <==
\pgfplotscreateplotcyclelist{corporate colours markers}{%
rot, every mark/.append style={fill=.!80!rot},mark=*\\%
mittelblau, every mark/.append style={fill=.!80!mittelblau},mark=square*\\%
apfelgruen, every mark/.append style={fill=.!80!apfelgruen},mark=triangle*\\%
orange, mark=star\\%
pink, every mark/.append style={fill=.!80!pink},mark=diamond*\\%
violettblau, every mark/.append style={fill=.!80!violettblau},mark=otimes*\\%
lila, mark=|\\%
gelb, every mark/.append style={fill=.!80!gelb},mark=pentagon*\\%
hellgrau, mark=text,text mark=p\\%
anthrazit, mark=text,text mark=a\\%
}

\pgfplotscreateplotcyclelist{corporate colours markers double}{%
rot, every mark/.append style={fill=.!80!rot},mark=*\\%
rot, dashed, every mark/.append style={fill=.!80!rot,solid},mark=*\\%
mittelblau, every mark/.append style={fill=.!80!mittelblau},mark=square*\\%
mittelblau, dashed, every mark/.append style={fill=.!80!mittelblau,solid},mark=square*\\%
apfelgruen, every mark/.append style={fill=.!80!apfelgruen},mark=triangle*\\%
apfelgruen, dashed, every mark/.append style={fill=.!80!apfelgruen,solid},mark=triangle*\\%
orange, mark=star\\%
orange, dashed, mark=star\\%
pink, every mark/.append style={fill=.!80!pink},mark=diamond*\\%
pink, dashed, every mark/.append style={fill=.!80!pink,solid},mark=diamond*\\%
violettblau, every mark/.append style={fill=.!80!violettblau},mark=otimes*\\%
violettblau, dashed, every mark/.append style={fill=.!80!violettblau,solid},mark=otimes*\\%
lila, mark=|\\%
lila, dashed, mark=|\\%
gelb, every mark/.append style={fill=.!80!gelb},mark=pentagon*\\%
gelb, dashed, every mark/.append style={fill=.!80!gelb,solid},mark=pentagon*\\%
}
